Probabilistic Obstruction Temporal Logic: a Probabilistic Logic to Reason about Dynamic Models

In this paper, we propose a novel formalism called Probabilistic Obstruction Temporal Logic (POTL), which extends Obstruction Logic (OL) by incorporating probabilistic elements. POTL provides a robust framework for reasoning about the probabilistic behaviors and strategic interactions between attackers and defenders in environments where probabilistic events influence outcomes. We explore the model checking complexity of POTL and demonstrate that it is not higher than that of Probabilistic Computation Tree Logic (PCTL), making it both expressive and computationally feasible for cybersecurity and privacy applications.

==> Properties.tex <==
\section{Main Properties}\label{sec:properties}
In this section, we first prove some remarkable semantic equivalences between \abbrv{POL} formulas. We then show that the satisfaction relation and the memoryless satisfaction relation coincide. Before we start, let us first define the obstruction predecessor operator. The obstruction predecessor of a set of states $A$, denoted $\blacktriangledown(n, A)$, is defined as the set of states that characterizes all predecessors of the set of states $A$, where each state $q$ $\in$ $A$ satisfies $\blacktriangleright(q, n, \overline{A)}$, that is, it can transition to a state not in the set $A$ where the sum of all successors of $q$ is less than or equal to $n$. 
%Intuitively, a state s belongs to (n, S) when the Demon can ensure that all action available to S that inevitably leads to a state that is not in S can be erased.

\begin{definition}[Obstruction Predecessor]
  Let $\mathcal{M}=(Q, q_0, \mathbf{P}, \mathcal{L}, \mathsf{C})$ be a model. %We recall that if $s$ is a state $post(s)$ and $pre(s)$ denote, respectively, the set of successors of $s$ and the set of predecessors of $s$. Given a set of states $A$, we define $Pre(A)=\bigcup_{s\in A} pre(s)$. 
Given a state  $q$,  a natural number $n$, and  a set of states $A$, we write:

$$\blacktriangleright(q,n,A) \ = \ \sum_{q'\in A} \mathsf{C}(q,q')\leq n $$ 
$$\blacktriangledown(n,A) =  \set{q \in \abbrv{Pre}(A) \, \mid \,  \blacktriangleright(q,n,\overline{A})}$$

\end{definition}

%Given a finite \abbrv{POS} $\mathcal{M}$, state $s$ in $\mathcal{M}$, and \abbrv{POL} state formula $\varphi$, determine whether $\mathcal{M}, q \models \varphi$. As for \abbrv{OL} model checking, the basic procedure is to compute the satisfaction set $\abbrv{Sat}(\varphi)$. Let $\varphi$ be any formula, then \abbrv{Sat}$({\varphi})$ denotes the set of states of $\mathcal{M}$  verifying, $\varphi$, i.e., \abbrv{Sat}$(\varphi)=\set{q \in Q \ \, | \, \ \mathcal{M}, s \models \varphi}$. The most interesting part of our logic is the treatment of the formula  $\psi$ = $\langle  {\sabotage_n}^{\bowtie k} \rangle  \theta$.
 %Let $\varphi$ be any formula:  $\sem{\varphi}^\M$ denotes the set of states of $\M$ verifying, $\varphi$, i.e., $\sem{\varphi}^\M=\set{s\in S \, : \,  \M,s\models \varphi}$. We omit the superscript $\M$ when the model is clear from the context. 
% In order to determine whether $q$ $\in$ $\abbrv{Sat}(\psi)$,  we will use $\abbrv{Pr}_{\mathcal{M}, q}^{\strat}$ $(\theta)$ to denote the probability that a path from $q$ satisfies path formula $\theta$ under n-strategy $\strat$: $\abbrv{Pr}_{\mathcal{M}, q}^{\strat}(\theta) = \abbrv{Pr}_{q}^{\strat}(\{\pi \in  \abbrv{Paths}_{\mathcal{M}, q}^{*}  \mid \mathcal{M}, \pi \models \theta \})$. Then  
% $$\abbrv{Sat}(\psi) = \{q \in Q \ \mid \  \abbrv{Pr}_{\mathcal{M}, q}^{\strat}(\theta) \bowtie k \}.$$

%We omit the superscript $\mathcal{M}$ in $\abbrv{Pr}_{q}^{\strat}$ $(\theta)$ when the model is clear from the context. We are now ready to characterize the set of states satisfying a formula $\langle{\sabotage_n}^{\bowtie k}\ \rangle \prox \varphi$.

\begin{proposition}\label{prop:1}
    For every model $\mathcal{M}$, state $q$, and formula $\varphi$ we have that  $q$ $\in$ $\langle{\sabotage_n}^{\bowtie k}\ \rangle \prox \varphi$ if and only if $q \in \blacktriangledown{(n,  \abbrv{Sat}(\varphi))}$. 
\end{proposition}
\begin{proof}

For the  $(\Rightarrow)$-direction:  suppose that $q \in \abbrv{Sat}(\langle{\sabotage_n}^{\bowtie k} \rangle$ $\prox \varphi)$, thus there is a n-strategy $\strat$  such that for all $\pi\in Out(s,\strat)$ we have that $\M,\pi_2 \models \varphi$. Suppose, to reach a contradiction, that $s\notin \blacktriangledown(n,\sem{\varphi})$. This could either mean that $s\not\in Pre(\varphi)$ or that $s\in Pre(\varphi)$ and that $\sum_{s'\in \overline{\sem{\varphi}}}\mathsf{C}(s,s') > n$. In the first case, we immediately obtain a contradiction. In the second case, we remark that any n-strategy can deactivate a subset of directed edges whose cost is at most $n$. Thus given any n-strategy $\strat'$ there is a path $\pi \in Out(s,\strat')$ such that $\pi_2\in \overline{\sem{\varphi}}$, which contradicts that $\M,s\models \naww{\sabotage_n}\next\varphi$. 
 	
For the  $(\Leftarrow)$-direction:  suppose that $s \in \blacktriangledown(n,\sem{\varphi})$. By definition, this means that $s\!\in\! Pre(\sem{\varphi})$  and that if $e_1,\ldots,e_n$ are all the edges from $s$ to $\overline{\sem{\varphi}}$, then $(\mathsf{C}(e_1) + \cdots + \mathsf{C} (e_n)) \!\leq\! n$.
Thus, a n-strategy verifying $\naww{\sabotage_n}\next \varphi$ is readily obtained by selecting the set $\set{e_1,\ldots, e_n}$ given the history $h=s$, and the empty-set for any other history $h'$.  
\end{proof}

In the next proposition, we provide the fix-point characterization for the OL operators. 

\begin{proposition}\label{lemma:1}
    For any two formulae $\varphi$ and $\psi$ we have that: 
    \begin{enumerate}
       \item\label{equiv:2} $\naww{\sabotage_n}(\varphi \until \psi)\equiv \psi \vee (\varphi \land \naww{\sabotage_n}\next( \naww{\sabotage_n}(\varphi \until \psi)))$;
       \item\label{equiv:1} $\naww{\sabotage_n} (\varphi \release \psi) \equiv \psi \land  (\varphi \vee  \naww{\sabotage_n} \next (\naww{\sabotage_n} (\varphi \release \psi)))$.
    \end{enumerate}
\end{proposition}
\begin{proof}
 We only prove~(\ref{equiv:2}), the proof of~(\ref{equiv:1}) being entirely similar. 
 
 %\begin{itemize}
 %\item[] 
 $(\Rightarrow)$
 Suppose that $\M,s \models \naww{\sabotage_n} (\varphi \until \psi)$, thus there is a n-strategy $\strat$, such that for every $\tau\in Out(s,\strat)$ there is a $j\in \mathbb{N}$ such that $\M,\tau_j \models \psi $ and $\M,\tau_k \models \varphi$ for every $1\leq k < j$.  If $\M, s \models \psi$ then we can conclude, otherwise since $s=\tau_1$ for any $\tau\in Out(s,\strat)$, we must have that $\M,s\models \varphi$ by hypothesis. Consider the n-strategy $\strat'$ defined by: 
 \begin{equation*}
     \strat'(h)= \begin{cases}
        \strat(h') & \text{if $h'=sh$ and $h'\sqsubset \tau $ for $\tau\in Out(s,\strat)$} \\
        \emptyset & \text{otherwise}.
     \end{cases}
 \end{equation*}
 
  Let $\mathcal{C}=\set{s' \, : \,  \exists \tau \in Out(s,\strat) \text{ s.t. } \tau_2=s'}$; 
	 given any $s'\in \mathcal{C}$  we clearly have that  $\rho \models \varphi \until \psi $ for any $\rho\in Out(s',\strat')$. We deduce that $\M,s'\models \naww{\sabotage_n} \varphi \until \psi$ (the Demon can use the above defined n-strategy $\strat'$) and since the Demon can get to any of the $s'$ by disabling the successors of $s$ disabled by $\strat$ we conclude that $\M, s \models \naww{\sabotage_n} \next ( \naww{\sabotage_n} (\varphi \until \psi))$. 	
	
	
	
 %\item[]
 $(\Leftarrow)$ Suppose that $\M,s \models \psi \vee (\varphi \land \naww{\sabotage} \next (\naww{\sabotage}(\varphi \until \psi )))$. If $\M,s \models \psi$ then we can conclude.  Otherwise $\M,s \models \varphi$ and $\M,s \models \naww{\sabotage_n} \next (\naww{\sabotage_n}(\varphi \until \psi ))$. By the definition of satisfaction, this means that there  is a  n-strategy $\strat$ such that $\M,\rho_2 \models \naww {\sabotage} \varphi \until   \psi $ for any $\rho\in Out(s,\strat)$.  By applying again the definition of satisfaction, we get that there is a n-strategy $\strat_{\rho_2}$ such that for every $\tau\in Out(\rho_2, \strat_{\rho_2}) $ we have that $\M, \tau_k  \models \psi$ for some $k\geq 1$ and $\M,\tau_j \models \varphi$ for any $1\leq j  < k$. 
 We define another n-strategy $\strat''$ by 

 \begin{equation*}
     \strat''(h)= 
     \begin{cases}
         \strat(h) & \text{if $h=s$}\\
         \strat_{\pi_2}(h') & \text{if $h'=s h$ and $h \sqsubset \tau$ for} \\ & \text{$ \tau\in Out(\pi_2,\strat_{\pi_2})$ and $\pi\in Out(s,\strat)$} \\
         \emptyset & \text{otherwise}
     \end{cases}
 \end{equation*}
 
   By the definition of $\strat''$, we obtain that $s\rho\in Out(s,\strat'')$ implies $\rho\in Out(s,\strat_{\pi_2})$ for some $\pi \in Out (s, \strat)$.  Now: suppose that there is a $\tau\in (s,\strat'')$ such that (1)  $\M, \tau_j \not\models \psi$ for all $j\in \mathbb{N}$ or  such that  (2)  $\M, \tau_k \models \psi$ for  some $k\in \mathbb{N}$, and there is a $1 \leq j < k$ such that $\M, \tau_j \not \models \varphi$. In both cases we get a contradiction because such a path also belongs to $Out(\pi_2,\strat_{\pi_2})$ for some $\pi\in Out(s,\strat)$. We can thus finally conclude that $\M,s\models \naww{\sabotage_n} (\varphi \until \psi)$ as we wanted. 
 %\end{itemize}
\end{proof}



Let $\M=\tuple{S,R, \mathcal{L},\mathcal{C}}$ be a model and $\varphi$, $\psi$ be two formulae. Consider the two monotone functions $\mathsf{R^n}_{\varphi,\psi}$ and $\mathsf{U^n}_{\varphi,\psi}$ from $2^S$ to itself, for any subset $X$ of $S$, defined by: 
\begin{equation}
    \mathsf{U}^n_{\varphi,\psi}(X)  = \sem{\psi}^\M \cup (\sem{\varphi}^\M \cap \blacktriangledown (n, X)) 
\end{equation}
\vspace{-2em}
\begin{equation}\label{eq:release}
    \mathsf{R}^n_{\varphi,\psi}(X)  = \sem{\psi}^\M \cap (\sem{\varphi}^\M \cup \blacktriangledown (n, X)) 
\end{equation}
\noindent we can prove the following. 

\begin{thm}\label{thm:fixpoint}
    For every model $\M$ and two formulae $\varphi$ and $\psi$: 
    \begin{enumerate}
        \item\label{fixpoint:2} $\sem{\naww{\sabotage_n} (\varphi \until \psi)}^\M$ is the least fix-point of  $\mathsf{U}^n_{\varphi,\psi}$;
        \item\label{fixpoint:1} $\sem{\naww{\sabotage_n} (\varphi \release \psi)}^\M$ is the greatest fix-point of $\mathsf{R}^n_{\varphi,\psi}$. 
    \end{enumerate}
\end{thm}
\begin{proof}
We only give a proof of~(\ref{fixpoint:1}). In virtue of Propositions~\ref{prop:1} and~\ref{lemma:1} it is clear that $X=\sem{\naww{\sabotage_n}(\varphi \release \psi)}^\M$ is a fix-point of $\mathsf{R}^n_{\varphi,\psi}$. Let $Y$ be any other fix-point of the function. If $Y=\emptyset$ the result trivially holds. Otherwise, we show that  given $v\in Y$ we have that  $v\in X$. Since $Y$ is a fix-point of the function, we have that $v\in \sem{\psi}$ and either  $v\in \sem{\varphi}$ or $v\in \blacktriangledown(n, Y)$. If this last case,  for the set  $E_v$ of edges whose source is $v$ and whose target is not in $Y$ we have that $(\sum_{e\in E_v} \mathcal{C}(e))\leq n$. We define an n-memoryless  strategy $\strat$ by 

\begin{equation*}
    \strat(v) = 
    \begin{cases}
         E_v & \text{ if } v\in \sem{\psi} \cap \blacktriangledown (n,Y) \\
         \emptyset & \text{ otherwise}
    \end{cases}
\end{equation*}

Now consider a path $\rho\in  Out(v,\strat)$ for $v\in Y$.   %By construction of $\strat$, we have that for any $i\in \mathbb{N}$, $\rho_i \in Y$ implies that either $\rho_i \in {\varphi}^\M $ or $\rho_{i+1} \in \sem{\psi}$.
Since $\rho_1=v\in Y$, let $\mathcal{X}=\set{k\geq 2 \, : \, \rho_k\not\in Y}$. If $\mathcal{X}$ is empty, then each $\rho_i\in \sem{\psi}$, otherwise let $j\geq 2$ be the smallest integer such that $\rho_j\not\in Y$. Suppose to reach a contradiction that $\rho_{j-1} \notin \sem{\varphi}$. Since $\rho_{j-1}\in Y$ and $\rho_j\notin \sem{\varphi}$ we must have that $\rho_j\in \sem{\psi} \cap \blacktriangledown (n,Y)$.   Thus, given any $\pi\in Out(\rho_j, \strat)$ we obtain that $\pi_2\in Y$. Since $\strat$ is memoryless, we obtain a contradiction  because $\pi_2=\rho_j$ for some $\pi \in Out(\rho_{j-1},\strat)$.  
\end{proof}



As we have anticipated, we now show that the set of formulae that are true under the satisfaction relation and the memoryless satisfaction relation coincides. 


\begin{lemma}
    For any formula $\varphi$, for any model $\M$ and state $s$: if $\M,s\models\varphi$ then $\M,s\models_{r}\varphi$.
\end{lemma}
\begin{proof}
    The proof is by induction on the structure of $\varphi$. Remark that for the case $\varphi=\naww{\sabotage_n} \psi_1\release \psi_2$, we showed in Theorem~\ref{thm:fixpoint} how given any $v$ belonging to a fix-point of the function~$\mathsf{R}^n_{\psi_1,\psi_2}$, it is possible to construct a n-memoryless strategy $\strat$ such that all paths in $Out(v,\strat)$ satisfies $\psi_1 \release \psi_2$. As a consequence, we only detail the cases $\varphi=\naww{\sabotage_n}\next \psi$ and $\varphi= \naww{\sabotage_n} (\psi_1 \until \psi_2)$. The proof for the $\naww{\sabotage_n} (\psi_1 \until \psi_2)$ case is inspired by the one presented in~\cite{KnapikPetrucciJamrogaTimed}. 
    %\begin{itemize}
        %\item 
        
    If $\varphi=\naww{\sabotage_n}\next \psi$, $\M,s\models \varphi$ iff there is a  n-strategy $\strat$ such that $\tuple{\M,\rho_2}\models \psi$ for all $\rho\in Out(s,\strat) $. By induction hypothesis, $\M,\rho_2 \models \psi$.  Consider the n-strategy $\strat'$ such that $\strat'(h)=\strat(s)$ if $last(h)=s$ and $\strat'(h)=\emptyset$ otherwise. This latter n-strategy is memoryless, and for any $\tau\in Out(s,\strat')$, $\tau_2=\rho_2$ which establish the wanted result. 
    \iffalse 
    if $\varphi=\naww{\sabotage_n}\globaly \psi$ then $\M,s\models \varphi$ iff there is a n-stratety $\strat$ s.t.  for any $i\in \mathbb{N}$, $\M, \rho_i \models \psi $ for every $\rho\in Out(s,\strat)$. Given an history $h=s_1,\ldots,s_n$ of $S$, we say that $h\in H^\strat_{s'}$ iff  $s_n=s'$, all the $s_i$ are distinct and $h\sqsubset \rho$ for some $\rho \in Out(s,\strat)$.  Given $H^\strat_{s'}$, we  choose one of its element that is minimal with respect to the prefix order, and denote it $h^{min}_{s'}$. We now define a memoryless n-strategy $\strat'$ by 
       \begin{equation*}
            \strat'(s') \begin{cases}
                \strat(h^{min}_{s'}) & \text{if $H^\strat_s\neq \emptyset$}
                \\
                \emptyset & \text{otherwise}
            \end{cases}
        \end{equation*}
        
        
         Let $h'$ be any finite sequence of states that is the prefix of some path in $Out(s,\strat')$;  we show that for any $i\leq |h|$,  $h_i=\rho_j$ for some $j\in \mathbb{N}$ and $\rho \in Out(s,\strat)$ by induction on $|h|$.
        If $|h'|=1$ then $h=s$ and  the result is clear. Suppose that the results holds for each $h''$ such that $|h''|\leq n$ and let $h'= s_1,\ldots,s_n, s_{n+1}$. If $s_{n+1}=s_i$ for some $i\leq n$, then we are done. Otherwise, $s_{n+1}$ is different from all the $s_i$. By definition, there is a path of the form  $\strat(h^{\min}_{s_n}), s_{n+1}$ over $S$, which implies that $s_{n+1}=\tau_j$ for some $\tau\in Out(s,\strat)$. 
\fi 
%\item

If $\varphi=\naww{\sabotage}\psi_1 \until \psi_2$. Let $\strat$ be a n-strategy such that $\psi_1 \until \psi_2$ holds for any path $\pi\in Out(s,\strat)$. Let $\mathcal{X}=\set{\pi_{\leq k} \, : \,  \pi \in Out(s,\strat) \land \M,\pi_k\models \psi_2 \land \M,\pi_j\models \psi_1 \text{ for all $1\leq j<k$} }$ and $\mathcal{Y}$ its prefix-closure.
Given  $v\in S$, let $h_v$  be a  sequence in  $\mathcal{Y}$ such that $last(h_v)=v$ and $\not\exists h^\star\in \mathcal{Y}$ such that $h_v\sqsubset h^\star$ and $last(h^\star)=v$. Define a n-strategy $\strat_{h_v}$ by: 
\begin{equation*}
    \strat_{h_v}(h)=\begin{cases} \strat(h_v\cdot h'') & \text{ if $h=h'\cdot h''$ and $last(h')=v$ }
    \\
    \strat(h) & \text{otherwise}
    \end{cases}
\end{equation*}
Such a n-strategy associates the same set of edges to any history ending in $v$ and we clearly have that  any path in its outcome set verifies $\psi_1 \until \psi_2$. Repeat the above procedure for any $s'\in S$. After at most $|S|$ steps, we obtain a memoryless n-strategy $\strat'$ in which any path verifies $\psi_1 \until \psi_2$. 
%\end{itemize}
\end{proof}
 By the above lemma and by the fact that any memoryless n-strategy is a n-strategy, one immediately obtains the following. 
\begin{thm}\label{thm:memoryless}
    For any formula $\varphi$, for every model $\M$ and state $s$, we have that  $\M,s\models_{r}$ if and only if $\M,s \models \varphi$.
\end{thm}

